Semantic-First: Temporal Scheduling in Flow Matching for Reliable Emotional Image Generation

Affect-controlled image generation should change how a scene feels while preserving what the prompt specifies. We study the temporal allocation of stochastic exploration and policy optimization in flow-matching models as a means of controlling this balance. During RL training, our semantic-first schedule uses deterministic ordinary differential equation (ODE) sampling during the high-noise phase and confines stochastic differential equation (SDE) exploration and group relative policy optimization (GRPO) to a late window. Controlled experiments separate exploration location, optimization location, and terminal-step sampling, showing distinct semantic benefits from late exploration and late updates. On FLUX.1-dev, semantic-first improves prompt faithfulness, independently evaluated affect accuracy, and human-rated semantic preservation and overall preference. The expanded semantic audit records 2.7% subject drift, while GRPO training time decreases by 41.1% relative to original full-path Flow-GRPO. Window-width experiments characterize the affect-semantic and computational trade-offs, and replication on SD3.5-Medium reproduces the scheduling advantage. These results establish denoising time as a practical control dimension for reliable emotional image generation.

==> highlights.tex <==
\begin{itemize}
\item Late-window scheduling preserves prompt semantics in affect-controlled generation.
\item Separate exploration and optimization controls identify temporal contributions.
\item Independent affect evaluation, TIFA, and expanded human auditing support the method.
\item Width tests and SD3.5-Medium replication extend the empirical evidence.
\item Eight-A100 training time falls by 41.1\% relative to original full-path training.
\end{itemize}

